From Rough Consensus to Automated Reasoning

Unwritten languages today often have no official grammar, and are rather governed by "unspoken rules". Similarly, we argue that the young discipline of networking is still a practice that lacks a deep understanding of the rules that govern it. This situation results in a tremendous loss of time and efforts. First, since the rules are unspoken, they are not systematically reused. Second, since there is no grammar, it is impossible to assert if a sentence is correct. Comparing two networking approaches or solutions is sometimes a synonym of endless religious debates. Drawing the proper conclusion from this claim, we advocate that networking research should spend more efforts on better understanding its rules as a first step to automatically reuse them. To illustrate our claim, we focus in this paper on one specific networking problem, and show how different instances of this same problem were solved in parallel, resulting in different solutions, and no explicit knowledge reuse.

==> related.tex <==
\section{Related work}\label{related}
Related work can be divided into two main families: (1) building networking operating systems and programming languages, and (2) enabling network programmability by separating control and data planes.

==> section3.tex <==
\section{Today's Networking axioms}\label{axiomas}
Develop here what are the axioms of networking today? 

End hosts are physically connected through dedicated network elements.\\
Both end hosts and network elements have certain capabilities:\\
\begin{itemize}
	\item End hosts have processing, memory and networking capabilities. Humans instrument end hosts to produce, process and store information. End hosts have networking interfaces which can generate information on the wire. Information is named (e.g. filename, URL). Network interfaces are named (MAC addresses, IP addresses). Hosts are also named (IP adresses) and Programs running ( 
	\item Networking elements have a set of named networking interfaces. They receive signals as an input from one interface, and produce a signal as an output to one or more interfaces. They have evolved through history to acquire more and more capabilities. From the basic hub functionality (take from one interface and send to all interfaces) all the way long till openflow's generic match and action switching.
\end{itemize}

\section{Networking knowledge representation}\label{representation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Each protocol applies on a given network configuration and results in a set of processing rules that the network elements execute.

At a first level, the problem starts with a set of end hosts with given networking capabilities with no physical connection between them. The first aspect is to guess what physical connections to do between the hosts, where to place network elements, and what processing they should do.

At a second level, given a certain physical connection, and network elements with their capabilities, the next step is what protocols to activate in order to get what we need. For example, an IGP results in a routing table for which each networking element has a route to each networking element in its domain. MPLS gives in addition...  BGP MPLS gives in addition...

\section{Use case study}\label{usecase}
Once we progress our understanding of the above mentioned issues, we need to apply the yet to be defined reasonner on some of the problems for which we have solutions today (e.g. the VPN problem, the data center problem etc.). We need then to compare the solution that the ``reasonner'' found with the one(s) that the community found.


